Another Round of Breaking and Making Quantum Money: How to Not Build It from Lattices, and More

Public verification of quantum money has been one of the central objects in quantum cryptography ever since Wiesner's pioneering idea of using quantum mechanics to construct banknotes against counterfeiting. So far, we do not know any publicly-verifiable quantum money scheme that is provably secure from standard assumptions. In this work, we provide both negative and positive results for publicly verifiable quantum money. **In the first part, we give a general theorem, showing that a certain natural class of quantum money schemes from lattices cannot be secure. We use this theorem to break the recent quantum money scheme of Khesin, Lu, and Shor. **In the second part, we propose a framework for building quantum money and quantum lightning we call invariant money which abstracts some of the ideas of quantum money from knots by Farhi et al.(ITCS'12). In addition to formalizing this framework, we provide concrete hard computational problems loosely inspired by classical knowledge-of-exponent assumptions, whose hardness would imply the security of quantum lightning, a strengthening of quantum money where not even the bank can duplicate banknotes. **We discuss potential instantiations of our framework, including an oracle construction using cryptographic group actions and instantiations from rerandomizable functional encryption, isogenies over elliptic curves, and knots.

==> instantiations_gather.tex <==
\section{Instantiations For Invariant Quantum Money}
\label{sec:instantiations_gather}



==> invariant.tex <==
\section{Invariant Money Correctness, Assumptions and Security}
\label{sec:invariant_append}


In this section, we fill in the proofs needed for the invariant quantum money scheme in Section \ref{sec:invariant_main}.
We will sometimes restate some theorems and remarks for the clarity of presentation.

\iffalse
We now describe our framework for instantiating quantum money using invariants, or more precisely what we call \emph{walkable} invariants. Let $X,Y$ be sets, and $I:X\rightarrow Y$ an efficiently computable function from $X$ to $Y$. $I$ will be called the ``invariant.'' We will additionally assume a collection of permutations $\sigma_i:X\rightarrow X$ indexed by $i\in [r]$ for some integer $r$, with the property that the permutations respect the invariant:
\[I(\;\sigma_i(x)\;)=I(x)\forall i\in[r]\]
In other words, action by each $\sigma_i$ preserves the value of the invariant. We require that $\sigma_i$ is efficiently computable given $i$. $r$ may be polynomial or may be exponential. To make the formalism below simpler, we will be implicitly assuming that there exists a perfect matching between the $\sigma_i$ such that for any matched $\sigma_i,\sigma_{i'}$, we have $\sigma_{i'}=\sigma_{i}^{-1}$. Moreover, $i'$ can be found given $i$. This can be relaxed somewhat to just requiring that $\sigma_i^{-1}$ can be efficiently computed given $i$, but requires a slightly more complicated set of definitions.

Given a point $x$, the orbit of $x$, denoted $O_x\subseteq X$, is the set of all $z$ such that there exists a non-negative integer $k$ and $i_1,\dots,i_k\in[r]$ such that $z=\sigma_{i_k}(\sigma_{i_{k-1}}(\cdots\sigma_{i_1}(x)\cdot ))$. In other words, $O_x$ is the set of all $z$ ``reachable'' from $x$ by applying some sequence of permutations. Note that $I(z)=y$ for any $z\in O_x$. We will therefore somewhat abuse notation, and define $I(O_x)=y$. We also let $P_y$ be the set of pre-images of $y$: $P_y=\{x\in X:I(x)=y\}$.

We will additionally require a couple properties, which will be necessary for the quantum money scheme to compile:
\begin{itemize}
	\item {\bf Efficient Generation of Superpositions:} It is possible to construct the uniform superposition over $X$: $|X\rangle:=\frac{1}{\sqrt{|X|}}\sum_{x\in X}|x\rangle$.
	\item {\bf Mixing Walks:} For an orbit $O$, with a slight abuse of notation let $\sigma_{O,i}$ be the (possibly exponentially large) permutation matrix associated with the action by $\sigma_i$ on $O$. Then let $M_O=\frac{1}{r}\sum_{i\in[r]} \sigma_{O,i}$ be the component-wise average of the matrices. Let $\lambda_1(O),\lambda_2(O)$ be the largest two eigenvalues by absolute value\footnote{They are real-valued, since $M_O$ is symmetric, owing to the fact that we assumed the $\sigma_i$ are perfectly matched into pairs that are inverses of each other.}, counting multiplicities. Note that $\lambda_1(O)=1$, with corresponding eigenvector the all-1's vector. We need that there is an inverse polynomial $\delta$ such that, for every orbit $O$, $\lambda_2(O)\leq 1-\delta$. This is basically just a way of saying that a random walk on the orbit using the $\sigma_i$ mixes in polynomial time. 
\end{itemize}
We call such a structure above a walkable invariant.

\subsection{Quantum Money from Walkable Invariants}
\label{sec:qm_scheme_invariant}

We now describe the basic quantum money scheme

\paragraph{Minting.} To mint a note, first construct the uniform superposition $|X\rangle$ over $X$. Then apply the invariant $I$ in superposition and measure, obtaining a string $y$, and the state collapsing to:
\[|P_y\rangle:=\frac{1}{\sqrt{|P_y|}} \sum_{x\in P_y}|x\rangle\]
This is the quantum money state, with serial number $y$.

\paragraph{Verification.} To verify a supposed quantum money state $|\phi\rangle$ with serial number $y$, we do the following.
\begin{itemize}
	\item First check that the support of $|\phi\rangle$ is contained in $P_y$. This is done by simply applying the invariant $I$ in superposition, and measuring if the output is $y$. If the check fails immediately reject.
	\item Then apply the projective measurement given by the projection $\sum_{O\subseteq P_y}|O\rangle\langle O|$, where $O$ ranges over the orbits contained in $P_y$, and $|O\rangle:=\frac{1}{\sqrt{|O|}}\sum_{x\in O}|x\rangle$. In other words, project onto states where, for each orbit, the weights of $x$ in that orbit are all identical; weights between different orbits are allowed to be different.
	
	We cannot perform this measurement exactly, but we can perform it approximately using the fact that $\lambda_2(O)\leq 1-\delta$. This is described in Section~\ref{sec:verification} below. Outside of Section~\ref{sec:verification}, we will assume for simplicity that the measurement is provided exactly.
	
	If the projection rejects, reject the quantum money state. Otherwise accept.
\end{itemize}

It is hopefully clear that honestly-generated money states pass verification. Certainly their support will be contained in $P_y$, and they apply equal weight to each element in an orbit (and in fact, equal weight across orbits).

\fi




\subsection{Approximate Verification}
\label{sec:verification}

%Here, we explain how to approximately perform the verification projection $V=\sum_{O\subseteq P_y}|O\rangle\langle O|$, using the fact that $\lambda_2(0)\leq 1-\delta$ for all $O$. The algorithm we provide is an abstraction of the verification procedure of~\cite{ITCS:FGHLS12}, except that that work presented the algorithm without any analysis. We prove that the algorithm is statistically close to the projection $V$, provided the mixing condition $\lambda_2(0)\leq 1-\delta$ is met.

\begin{theorem}\label{thm:verification}Assume $\lambda_2(0)\leq 1-\delta$ for all $O$, for some inverse-polynomial $\delta$. Then there is a QPT algorithm $\tilde{V}$ such that, for any state $|\psi\rangle$, if we let $|\psi'\rangle$ be the un-normalized post-measurement state from applying $\tilde{V}$ to $|\psi\rangle$ in the case $\tilde{V}$ accepts, then $|\psi'\rangle$ is negligibly close to $V|\psi\rangle$.\end{theorem}
Since the probability of acceptance for $\tilde{V}$ and $V$ just $\langle\psi'|\psi'\rangle$ and $\langle\psi|V|\psi\rangle$ respectively, this means the acceptance probabilities are negligibly close. Moreover, with overwhelming probability, the post-measurement states (conditioned on verification) will be negligibly close.

\input{invariant_verification}



\iffalse
\begin{proof}Let $r'=2r$. Let $\Rs$ be a register containing a superposition over $1,\dots,r'$, and $\Ss$ be the register containing the supposed quantum money state. Define the following:
\begin{itemize}
	\item The unitary $U$ acting on $\Rs\otimes\Ss$ defined as $U=\sum_{i=1}^r |i\rangle\langle i|\otimes \sigma_i + \sum_{i=r+1}^{r'} |i\rangle\langle i|\otimes \Id$. Here, we use a slight abuse of notation, using $\sigma_i$ to denote the unitary implementing the classical permutation $\sigma_i$. $U$ can be computed efficiently, by our assumption that we can efficiently invert $\sigma_i$.
	\item The state $|\onev\rangle=\frac{1}{\sqrt{r'}}\sum_{i=1}^{r'}|i\rangle$
	\item The projection $P=|\onev\rangle\langle\onev|\otimes\Id$. 
\end{itemize}

\noindent Our algorithm is the following:
\begin{itemize}
	\item Initialize the register $\Rs$ to $|\onev\rangle$.
	\item Repeat the following $t=\lambda/\delta$ times:
	\begin{itemize}
		\item Apply the unitary $U$ to $\Rs\otimes\Ss$.
		\item Apply the measurement corresponding to projection $P$ to $\Rs\otimes\Ss$. If the measurement outcome is reject, immediately abort and reject the state.
		\item Apply $U^{-1}$.
	\end{itemize}
	\item If all $t$ trials above accepted, then accept and output the contents of the $\Ss$ register.
\end{itemize}

We now analyze the algorithm above. $M=\frac{1}{r}\sum_{i\in[r]} \sigma_i$. This matrix is symmetric, since we assumed the $\sigma_i$ come in pairs that are inverses of each other. It is not necessarily positive. For example, consider $X$ that can be divided into two subsets $X_0,X_1$ such that each $\sigma_i$ maps $X_b$ to $X_{1-b}$. Then the vector that places equal weight on all $x\in X$, but makes the values in $X_0$ positive and $X_1$ negative will have eigenvalue $-1$. In general, the eigenvalues of $M$ must be in the real interval $[-1,1]$. The eigenvectors with eigenvalue 1 are exactly $|O\rangle$ and the space spanned by them, as $O$ ranges over all possible orbits. By our mixing assumption, all other eigenvalues are at most $1-\delta$.

Suppose $|\psi_\ell\rangle$ is an eigenvector of $M$, with eigenvalue $\ell$. We now explore how the algorithm above behaves on $|\psi_\ell\rangle$. Then we will extend our understanding to non-eigenvector states.

We have that 
\begin{align*}
PU|\onev\rangle|\psi_\ell\rangle&=\frac{1}{\sqrt{r'}}\left(|\onev\rangle\langle\onev|\otimes\Id\right)\cdot\left(\sum_{i=1}^r |i\rangle\otimes \sigma_i|\psi_\ell\rangle + \sum_{i=r+1}^{r'} |i\rangle  |\psi_\ell\rangle\right)\\
&=\frac{1}{r'}|\onev\rangle\otimes\left(\sum_{i=1}^r \sigma_i |\psi_\ell\rangle+r |\psi_\ell\rangle\right)\\
&=|\onev\rangle\otimes\left(\frac{1}{2}M|\psi_\ell\rangle+\frac{1}{2}|\psi_\ell\rangle\right)=\left(\frac{1+\ell}{2}\right)|\onev\rangle|\psi_\ell\rangle
\end{align*}

Now consider a general state $|\psi\rangle$, which we write in an eigenbasis for $M$ as $|\psi\rangle=\sum_{\ell}\alpha_\ell|\psi_\ell\rangle$. Then $PU|\onev\rangle|\psi\rangle=\sum_{\ell}\alpha_\ell\left(\frac{1+\ell}{2}\right)|\psi_\ell\rangle$. After $t$ trials, we have:
\[(PU)^t|\onev\rangle|\psi\rangle=|\onev\rangle\otimes\sum_{\ell}\alpha_\ell\left(\frac{1+\ell}{2}\right)^t|\psi_\ell\rangle\]
Let $|\psi'\rangle$ be the state after discarding $|\onev\rangle$. Now
\begin{align*}|\enspace V|\psi\rangle-|\psi'\rangle\enspace |^2&=\left|\enspace|\psi_\ell\rangle-\sum_{\ell}\alpha_\ell \left(\frac{1+\ell}{2}\right)^t |\psi_\ell\rangle\enspace\right|^2\\
&=\left| -\sum_{\ell\neq 1}\alpha_\ell \left(\frac{1+\ell}{2}\right)^t |\psi_\ell\rangle\enspace\right|^2\\
&=\sum_{\ell\neq 1}|\alpha_\ell|^2 \left(\frac{1+\ell}{2}\right)^{2t}\\
&\leq \sum_{\ell\neq 1}|\alpha_\ell|^2 \left(1-\delta/2\right)^{2t}\\
&=(1-|\alpha_1|^2)\left(1-\delta/2\right)^{2t}\leq e^{-\lambda}
\end{align*}
This bound is negligible. This completes the proof of Theorem~\ref{thm:verification}.
\end{proof}
\fi



\input{invariant_assumptions} 

==> kLWE.tex <==
%!TEX root = ./Attacking.tex

\section{The~\cite{KLS22} $k$-LWE Problem Is Hard}
\label{sec:kLWE_old}

In this section we prove Lemma~\ref{lem:klwe}, showing that the $k$-LWE problem is hard, assuming the hardness of LWE. This will finish the proof that the states produced by our attack are indistinguishable from valid quantum money states. We begin by providing some basic definitions.  Then we prove some supplementary lemmas, and finally we prove the whole result.

\subsection{General LWE Definition}
We first provide a properly parameterized definition of the LWE problem~\cite{STOC:Regev05}. \textcolor{red}{Hart:  we don't need the full generality of this definition now but may need it if we want to generalize our argument.}

\begin{definition}~\label{def:LWE} \textbf{Learning with Errors (LWE) Problem:}
Let $n$, $m$, and $q$ be integers, let $\mathcal{D}_{\Am}$ and $\mathcal{D}_{\Sm}$ be distributions over $\Z_{q}^{n}$, and let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution over $\Z_{q}^{m}$.  Let $\Am \in \Z_{q}^{m \times n}$ be a matrix where each row is sampled from $\mathcal{D}_{\Am}$, let $\sv \in \Z_{q}^{n}$ be a vector sampled from $\mathcal{D}_{\Sm}$, and let $\mathbb{e} \in \Z_{q}^{m}$ be a vector sampled from $\mathcal{D}_{\mathbb{\Psi}}$.  Finally, let $\rv \in \Z_{q}^{m}$ be a uniformly random vector.

The $\left(n, m, q, \mathcal{D}_{\Am}, \mathcal{D}_{\Sm}, \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE problem is defined to be distinguishing between the following distributions: 
\[  \left( \Am, \Am \cdot \sv + \ev \right) \text{ and } \left( \Am, \rv \right) \] .
\end{definition}

In his seminal work~\cite{STOC:Regev05}, Regev showed that LWE was hard worst-case lattice problems for uniformly random choices of $\mathcal{D}_{\Am}$ and $\mathcal{D}_{\Sm}$ and when $\mathcal{\mathbb{\Psi}}$ was defined to be choosing each coordinate as a (small) discrete Gaussian.

\subsection{LWE with a ``Hint'' about the Secret Key}
The first step in our proof involves proving that LWE with a ``hint'' about the secret key is as hard as a slightly lower-dimensional version of LWE.  We define the problem below.  Note that we need to fix some of the distributions in the general LWE definition to be uniform for this lemma to be true, so we do that (at the expense of some generality) in our proof.  We also emphasize that this sort of result is not new and much more general statements than what we are proving are possible (for instance, see~\cite{goldwasser2010robustness}), but we find it useful to prove a precisely tailored version of our statement.

We begin by defining our precise problem statement.

\begin{definition}~\label{def:LWEHint} \textbf{LWE with a Hint Problem:}
Let $n$, $m$, and $q$ be integers, let $\mathcal{D}_{\Am}$ and $\mathcal{D}_{\Sm}$ be distributions over $\Z_{q}^{n}$, and let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution over $\Z_{q}^{m}$.  Let $\Am \in \Z_{q}^{m \times n}$ be a matrix where each row is sampled from $\mathcal{D}_{\Am}$, let $\sv \in \Z_{q}^{n}$ be a vector sampled from $\mathcal{D}_{\Sm}$, and let $\ev \in \Z_{q}^{m}$ be a vector sampled from $\mathcal{D}_{\mathbb{\Psi}}$.  Finally, let $\rv \in \Z_{q}^{m}$ and $\cv \in \Z_{q}^{m}$ be uniformly random vectors.

The $\left(n, m, q, \mathcal{D}_{\Am}, \mathcal{D}_{\Sm}, \mathcal{D}_{\mathbb{\Psi}} \right)$-HintLWE problem is defined to be distinguishing between the following distributions: 
\[  \left( \Am, \cv, \cv \cdot \sv,  \Am \cdot \sv + \ev \right) \text{ and } \left( \Am, \cv, \cv \cdot \sv, \rv \right) \] .
\end{definition}

We next prove that, for a particular instantiation (namely, when all but the noise distributions are uniform), the LWE with a hint problem is as hard as the LWE problem in one less dimension.  We formalize this stament below.

\begin{lemma}~\label{lem:LWEHintHard}
Let $n$, $m$, and $q$ be integers, and let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution over $\Z_{q}^{m}$.

Any adversary that can be used to solve the $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right),  \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE with a hint problem with advantage $\epsilon$ can be used to solve the $\left(n - 1, m, q, \mathcal{U} \left( \Z_{q}^{n - 1} \right),  \mathcal{U} \left( \Z_{q}^{n - 1} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE problem with advantage $\epsilon$.
\end{lemma}

\begin{proof}
Suppose we are given a $\left(n - 1, m, q, \mathcal{U} \left( \Z_{q}^{n - 1} \right),  \mathcal{U} \left( \Z_{q}^{n - 1} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE challenge, which consists of these parameters plus a tuple $\left( \Am \in \Z_{q}^{m \times n-1}, \tv \in \Z_{q}^{m} \right)$ where either $\tv = \Am \cdot \sv + \ev$ or $\tv = \rv$, for appropriately sampled parameters.  We will show how to generate a properly distributed LWE with a hint challenge so that if the original LWE challenge was ``real'', the LWE with a hint challenge is ``real'', and if the original challenge was ``random'', then the simulated one is ``random'' too.  This will allow us to build an advantage-preserving reduction.

Suppose we sample a uniformly random vector $\uv \in \Z_{q}^{m}$, a uniformly random vector $\cv \in \Z_{q}^{m}$, and a uniformly random integer $z$.  In addition, suppose we choose a matrix $\tilde{\Cm} \in \Z_{q}^{n - 1 \times n}$ and define $\Cm \in \Z_{q}^{n \times n}$ to be the vertical concatenation of $\tilde{\Cm}$ and $\cv$ (i.e. $\Cm = \left[ \begin{array}{c} \tilde{\Cm} \\ \hline \cv \end{array} \right]$) subject to the constraint that $\Cm$ is invertible.

 We set $\Am' = \left[ \Am || \uv \right] \cdot \Cm$, where ``$||$'' denotes horizontal concatenation.  We then set $\tv' = \tv + z \uv$.  We claim that the tuple $\left(\Am', \cv, z, \tv' \right)$ is an appropriately distributed LWE with a hint challenge.  We prove that this is the case separately for the ``real'' and ``random'' cases below.

\medskip

\noindent \textbf{The ``Random'' Case}:  In this instance, we assume that $\tv$ is a uniformly random vector, and we need $\tv'$ to also be uniformly random.  Note that $\tv'$ is indeed uniformly random since $\tv' = \tv + z \uv$ and everything we sample in the reduction is sampled independently of $\tv$.   Moreover, note that $\Am'$ and $\cv$ are distributed uniformly as required (with the uniformity of $\Am'$ relying on the fact that $\Cm$ is invertible), and, since $\sv$ is uniformly random and independent of everything else given in the tuple, $\cv \cdot \sv$ will also be distributed statistically close to uniformly random\footnote{It's not exactly uniform due to the highly unlikely possibility that $\cv$ is the all zeroes vector.}, so sampling $z$ uniformly at random gives an appropriate tuple. 

\medskip

\noindent \textbf{The ``Real'' Case}:  In this case, we assume that $\tv = \Am \cdot \sv + \ev$.  We need to generate a ``real'' LWE with a hint challenge tuple. 

Note that 
\[
\tv' = \left[\Am || \uv \right] \cdot  \left[ \begin{array}{c} \sv \\ \hline z \end{array} \right] + \ev .
\]
We can write this as 
\[
\tv' = \left( \left[\Am || \uv \right] \cdot \Cm \right) \cdot \left( \Cm^{-1} \cdot  \left[ \begin{array}{c} \sv \\ \hline z \end{array} \right] \right) + \ev .
\]
Now suppose we set 
\[
\Am' =  \left[\Am || \uv \right] \cdot \Cm \text{ and } \sv' =  \Cm^{-1} \cdot  \left[ \begin{array}{c} \sv \\ \hline z \end{array} \right] 
\]
Due to the invertibility of $\Cm$ (and, by corollary, $\Cm'$) we know that both $\Am'$ and $\sv'$ are distributed uniformly at random as required.  Moreover, we have
\[
\cv^{T} \cdot \sv' = \cv^{T} \cdot \left( \Cm^{-1} \cdot  \left[ \begin{array}{c} \sv \\ \hline z \end{array} \right]  \right) = z
\]
as required.  Since we have sampled $\cv$ uniformly at random, we thus know that the tuple $\left(\Am', \cv, z, \tv' \right)$ is distributed as a proper LWE with a hint challenge in the ``real'' case as well, which lets us complete the proof.
\end{proof}

\subsection{The $k$-LWE Problem}
With all of the necessary background in place, we are ready to move to the actual $k$-LWE problem.  We first define the problem and then show that the variant of $k$-LWE implied by the~\cite{KLS22} construction is as hard as the LWE with a hint problem.  The $k$-LWE problem was first formally defined in~\cite{C:LPSS14} and used to build traitor-tracing schemes.  It extends $k$-SIS assumption~\cite{PKC:BonFre11} which was used to build linearly homomorphic signatures.  Our definition below is essentially a parameterized version of the one in~\cite{C:LPSS14}.

\begin{definition}~\label{def:kLWE} \textbf{$k$-LWE Problem:}
Let $k$, $n$, $m$, and $q$ be integers, let $\mathcal{D}_{\Sm}$ be a distribution over $\Z_{q}^{n}$, and let $\mathcal{D}_{\mathbb{\Psi}}$ and $\mathcal{D}_{\Km}$ be distributions over $\Z_{q}^{m}$.  Let $\Km \in \Z_{q}^{k \times m}$ be a matrix where each \emph{row} is selected from $\mathcal{D}_{\Km}$.  

Let $\Am \in \Z_{q}^{m \times n}$ be a matrix sampled uniformly from the set of matrices such that $\Km \cdot \Am = 0 \mod q$, let $\sv \in \Z_{q}^{n}$ be a vector sampled from $\mathcal{D}_{\Sm}$, and let $\mathbb{e} \in \Z_{q}^{m}$ be a vector sampled from $\mathcal{D}_{\mathbb{\Psi}}$.  Let $\Cm \in \Z_{q}^{m \times m - k}$ be a basis for the set of vectors $\vv \in \Z_{q}^{m}$ such that $\vv^{T} \cdot \Cm = 0$, and let $\sv' \in \Z_{q}^{m - k}$ be a uniformly random vector.

The $\left(k, n, m, q, \mathcal{D}_{\Km}, \mathcal{D}_{\Sm}, \mathcal{D}_{\mathbb{\Psi}} \right)$-$k$-LWE problem is defined to be distinguishing between the following distributions: 
\[  \left( \Km, \Am, \Cm, \Am \cdot \sv + \ev \right) \text{ and } \left(\Km, \Am,  \Cm, \Cm \cdot \sv' + \ev \right) \] .
\end{definition}

We note that $k$-LWE is traditionally defined in a slightly different way:  usually the matrix $\Am$ is sampled before (or jointly with) $\Km$ rather than after it.  We sample $\Km$ first in our definition because we will need to handle very unusual (at least for cryptographic applications) distributions $\mathcal{D}_{\Km}$.

\subsection{The~\cite{KLS22} $k$-LWE Distribution}
As we discussed earlier (and with slightly different notation), the $k$-LWE scheme implied by the~\cite{KLS22} scheme uses a matrix $\Km$ with the following distribution:
\begin{definition}~\label{def:KMat} \textbf{The~\cite{KLS22} Distribution Matrix $\Km$}: 
\[
\Km \in \Z_{q}^{3 \times m + 4} = \left[ \begin{array}{ccccccc}
2 \Gamma = 2t' + 1 & -2 & 0 & 0 & 0 & ... & 0 \\
0 & 1 & 1 & 0 & 0 & ... & 0 \\
0 & 0 & -2 & \Delta & 0 & ... & 0 
\end{array} \right]
\]
\end{definition}
We denote the rows of $\Km$ as $\Km_{1}$, $\Km_{2}$, and $\Km_{3}$, respectively.  Our choice of the number of columns in $\Km$ is arbitrary at this point, but these parameter choices will be useful later in our construction. Note that any vector $\vv \in \Z_{q}^{m + 4}$ such that $\Km \cdot \vv = 0 \mod q$ has the following form, where $c \in \Z_{q}$ is an integer and $\vv_{5}, ... , \vv_{m+4}$ are arbitrary:
\[
\vv = \left[ \begin{array} {l}
\vv_{1} = \left(2 \Delta \right) c \\
\vv_{2} = \left( \left(2t' + 1 \right) \Delta \right) c \\
\vv_{3} = \left( - \left(2t' + 1 \right) \Delta \right) c \\
\vv_{4} = \left( - 2 \left(2t' + 1 \right) \right) c \\
\vv_{5} \\
... \\
\vv_{m + 4}
\end{array} \right] .
\]

Additionally, note that any collection $\Vm \in \Z_{q}^{m + 4 \times n}$ of such vectors can be written as 
\[
\Vm = \left[ \begin{array}{c} 
\Xm \in \Z_{q}^{4 \times n} \\ \hline
\Ym \in \Z_{q}^{m \times n}
\end{array} \right]
\] 
for uniformly random $\Ym$ and for $\Xm$ with the following structure
\[
\Xm = \left[ \begin{array}{c}
2 \Delta  \\
\left(2t' + 1 \right) \Delta  \\
 - \left(2t' + 1 \right) \Delta  \\
- 2 \left(2t' + 1 \right)  \\
\end{array} \right] \cdot
\left[ \begin{array}{ccccc}
\cv_{1} & \cv_{2} & \cv_{3} & ... & \cv_{n} 
\end{array}\right]
\]
for $\cv_{i} \in \Z_{q}$.  Note that $\Xm$ is essentially just the tensor product of two vectors, one of which may be uniform ($\cv$) and one of which is extremely structured.

\subsection{$k$-LWE with the~\cite{KLS22} Distribution Is Hard}
We are now ready to prove our main result:  that $k$-LWE with the distribution defined by the~\cite{KLS22} construction is as hard as standard LWE.  To do this, we will work through the ``LWE with a Hint'' problem that we have defined earlier.  We formally state this as a lemma below.

\begin{lemma}~\label{lem:KLWEHint}
Let $n$, $m$, and $q$ be integers.  Let the matrix $\Km$ be defined as in definition~\ref{def:KMat}, and let $\mathcal{D}_{\Km}$ be the distribution that outputs the matrix $\Km$.  Let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution that is extensible to all vector lengths and outputs vectors where each entry is selected identically independently at random.

Any adversary that can solve the $\left(3, n, m + 4, q, \mathcal{D}_{\Km}, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-$k$-LWE problem with advantage $\epsilon$ can be used to solve the $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-HintLWE problem with advantage $\epsilon$.
\end{lemma}

\begin{proof}
Suppose that we are given an instance of the $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-HintLWE problem in the form of a tuple $\left( \Am, \cv, \cv \cdot \sv, \tv \right)$ where $\tv = \Am \cdot \sv + \ev$ or $\tv = \rv$ for some uniformly random $\rv$.  We will show how to transform this instance into a valid $k$-LWE instance such that if we started with a ``real'' instance of the LWE with a hint problem, we end up with a ``real'' instance of the $k$-LWE problem, and if we started with a ``random'' instance, we end up with a ``random'' instance.  This lets us build an advantage-preserving reduction.

Suppose we first (as above) define
\[
\Xm \in \Z_{q}^{4 \times n} = \left[ \begin{array}{c}
2 \Delta  \\
\left(2t' + 1 \right) \Delta  \\
 - \left(2t' + 1 \right) \Delta  \\
- 2 \left(2t' + 1 \right)  \\
\end{array} \right] \cdot
\left[ \begin{array}{ccccc}
\cv_{1} & \cv_{2} & \cv_{3} & ... & \cv_{n} 
\end{array}\right]
\]
and then set
\[
\Am' \in \Z_{q}^{m + 4 \times n} = \left[ \begin{array}{c} \Xm \\ \hline \Am \end{array} \right] .
\]
Let $e_{1}$, $e_{2}$, $e_{3}$, and $e_{4}$ be individual samples from $\mathcal{D}_{\mathbb{\Psi}}$.  We define a vector $\tv' \in \Z_{q}^{ m + 4 }$ in the following way:
\[
\tv' = \left[ \begin{array} {l}
\tv_{1}' = \left(2 \Delta \right) \cv \cdot \sv + e_{1} \\
\tv_{2}' = \left( \left(2t' + 1 \right) \Delta \right) \cv \cdot \sv + e_{2} \\
\tv_{3}' = \left( - \left(2t' + 1 \right) \Delta \right) \cv \cdot \sv + e_{3} \\
\tv_{4}' = \left( - 2 \left(2t' + 1 \right) \right) \cv \cdot \sv + e_{4} \\
\tv_{5}' = \tv_{1} \\
... \\
\tv_{m+4}' = \tv_{m}
\end{array} \right] .
\]
We claim that the tuple $\left( \Km, \Am', \Cm, \tv' \right)$ is a valid $k$-LWE tuple.  We will hande this in two cases--the ``real'' case and the ``random'' case--below. 

\medskip

\noindent \textbf{The ``Random'' Case}:  in this case, we are given a uniformly random $\tv$ and must show that our algorithm outputs $\tv' = \Cm \cdot \sv' + \ev'$.   Recall that every vector orthogonal to $\Km$ has the form 
\[
\vv = \left[ \begin{array} {l}
\vv_{1} = \left(2 \Delta \right) c \\
\vv_{2} = \left( \left(2t' + 1 \right) \Delta \right) c \\
\vv_{3} = \left( - \left(2t' + 1 \right) \Delta \right) c \\
\vv_{4} = \left( - 2 \left(2t' + 1 \right) \right) c \\
\vv_{5} \\
... \\
\vv_{m + 4}
\end{array} \right] .
\]
where $\vv_{5}, ... , \vv_{m + 4}$ could take any value.  Since $\cv \cdot \sv$ is distributed uniformly at random over $\Z_{q}$, we know that the vector 
\[
\left[ \begin{array} {l}
\left(2 \Delta \right) \cv \cdot \sv \\
\left( \left(2t' + 1 \right) \Delta \right) \cv \cdot \sv \\
\left( - \left(2t' + 1 \right) \Delta \right) \cv \cdot \sv  \\
\left( - 2 \left(2t' + 1 \right) \right) \cv \cdot \sv \\
\tv_{1} \\
... \\
\tv_{m}
\end{array} \right] 
\]
is distributed uniformly at random over the space of vectors orthogonal to $\Km$, which is the exact same distribution as $\Cm \cdot \sv'$.  Since the last $m$ entries of this vector are already uniform (and the noise is sampled independently for each entry) they are properly distributed even without the addition of any noise.  Thus, our distribution of $\tv'$ is correct.

Our previous paragraph can also be used to argue that our distribution of $\Am'$ is also correct, meaning that we have succesfully handled this case.

\medskip

\noindent \textbf{The ``Real'' Case}:  now, suppose we are given a value $\tv = \Am \cdot \sv + \ev$.  We need to show that our algorithm outputs $\tv' = \Am' \cdot \sv + \ev'$.  Note that, in this case we can write
\[
\tv' = \left[ \begin{array}{c} \Xm \\ \hline \Am \end{array} \right] \cdot \sv + \left[ \begin{array}{c}\ev' \\ \hline \ev \end{array} \right]
\]
for 
\[
\ev ' = \left[ \begin{array}{c}
e_{1} \\
e_{2} \\
e_{3} \\
e_{4}
\end{array} \right]
\]
which is the correct distribution for $\tv'$ in this instance.  This allows us to complete the proof.
\end{proof}

\subsection{Putting It All Together}
We can finally state a theorem about the hardness of $k$-LWE for the distribution implied by the~\cite{KLS22} scheme by combining our two main lemmas.  We do this as follows:

\begin{theorem}~\label{thm:schemeklwe}
Let $n$, $m$, and $q$ be integers.  Let the matrix $\Km$ be defined as in definition~\ref{def:KMat}, and let $\mathcal{D}_{\Km}$ be the distribution that outputs the matrix $\Km$.  Let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution that is extensible to all vector lengths and outputs vectors where each entry is selected identically independently at random.

Any adversary that can solve the $\left(3, n, m + 4, q, \mathcal{D}_{\Km}, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-$k$-LWE problem with advantage $\epsilon$ can be used to solve the $\left(n - 1, m, q, \mathcal{U} \left( \Z_{q}^{n - 1} \right),  \mathcal{U} \left( \Z_{q}^{n - 1} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE problem with advantage $\epsilon/2$.
\end{theorem}

\begin{proof}
This theorem follows from a simple hybrid argument over our two previous lemmas.
\end{proof}

We emphasize that this reduction preserves the distribution of the noise and almost preserves the dimensions of the problem.

==> kLWE2.tex <==
%!TEX root = ./Attacking.tex

\section{On the Hardness of $k$-LWE}
\label{sec:klwe}



In this section we prove a number of hardness results on $k$-LWE, showing that the $k$-LWE instance implied by the~\cite{KLS22} scheme is hard, assuming standard lattice assumptions.  In addition, we provide additional evidence through proofs that more general instances of $k$-LWE are likely to be hard, which seemingly indicates that it would be difficult to ``tweak'' the~\cite{KLS22} construction by altering the distributions to gain security.

We begin by providing some basic definitions.  Then we prove some supplementary lemmas, and finally we prove the whole result.

\subsection{Lattice Preliminaries}
We say a distribution $\mathcal{D}$ is $\left(B, \delta \right)$-bounded if the probability that $\mathcal{D}$ outputs a value larger than $B$ is less than $\delta$.  We extend this to distributions that output vectors in an entry-by-entry way.

We next define discrete Gaussians formally.  Since we later use their lemmas, our definition is loosely based on that of~\cite{STOC:BLPRS13}.

\begin{definition}~\label{def:discG}
For any $sigma > 0$, the $n$-dimensional Gaussian function $\rho_{\sigma} : \R^{n} \rightarrow \left[0, 1 \right]$ is defined as 
\[
\rho_{r} \left( \xv \right) = e^{ - \pi \frac{\xv^2}{\sigma^2}}
\]
We define the \emph{discrete Gaussian function} with parameter $\sigma$ at point $\pv \in \R^{n}$, which we usually denote $\mathcal{D}_{\mathbf{\Psi}_{\sigma}}$, as the function over all of the integers $\yv \in \Z^{n}$ such that the probability mass of any $\yv$ is proportional to
\[
e^{ - \pi \frac{\left( \pv - \yv \right)^2}{\sigma^2}} .
\]
\end{definition}

We define the GapSVP problem.

\begin{definition}~\label{def:GapSVP}
Let $n$ be an integer and $\gamma = \gamma \left(n \right) \geq q$ a real number.  The $\left(n, \gamma \right)$-GapSVP problem is the problem of deciding, given a basis $\Bm$ of an $n$-dimensional lattice $\Lambda$ and a number $d$, decide whether or not $\lambda_{1} \left( \Lambda \right) \leq d$ or $\lambda_{1} \left( \Lambda \right) > \gamma d$.
\end{definition}

We emphasize that GapSVP is a ``promise problem'' and that a (successful) adversary can output whatever it wants when $d < \lambda_{1} \left( \Lambda\ \right) \leq \gamma d$.

\subsection{Definitions}
In this section we define basic LWE and $k$-LWE.  We note that, while equivalent to the standard definitions, our definitions here are presented differently than usual in lattice cryptography.  This is so that we can keep the notation more consistent with the typical quantum money and quantum algorithms presentation styles.

\subsection{General LWE Definition}
We first provide a properly parameterized definition of the LWE problem~\cite{STOC:Regev05}. 

\begin{definition}~\label{def:LWE} \textbf{Learning with Errors (LWE) Problem:}
Let $n$, $m$, and $q$ be integers, let $\mathcal{D}_{\Am}$ and $\mathcal{D}_{\rv}$ be distributions over $\Z_{q}^{n}$, and let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution over $\Z_{q}^{m}$.  Let $\Am \in \Z_{q}^{m \times m}$ be a matrix where each row is sampled from $\mathcal{D}_{\Am}$, let $\rv \in \Z_{q}^{n}$ be a vector sampled from $\mathcal{D}_{\rv}$, and let $\ev \in \Z_{q}^{m}$ be a vector sampled from $\mathcal{D}_{\mathbb{\Psi}}$.  Finally, let $\tv \in \Z_{q}^{m}$ be a uniformly random vector.

The $\left(n, m, q, \mathcal{D}_{\Am}, \mathcal{D}_{\rv}, \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE problem is defined to be distinguishing between the following distributions: 
\[  \left( \Am,  \Am \cdot \rv + \ev \right) \text{ and } \left( \Am, \tv \right) . \] 
\end{definition}

In his seminal work~\cite{STOC:Regev05}, Regev showed that LWE was hard worst-case lattice problems for uniformly random choices of $\mathcal{D}_{\Am}$ and $\mathcal{D}_{\Rm}$ and when $\mathcal{\mathbb{\Psi}}$ was defined to be choosing each coordinate as a (small) discrete Gaussian.  To capture this, we cite a theorem from~\cite{STOC:BLPRS13} which itself is derived from Theorem 3.1 of~\cite{STOC:Regev05} and Theorem 3.1 of~\cite{STOC:Peikert09}.

\begin{theorem}~\label{thm:LWEHardness} \textbf{(Theorem 2.16,~\cite{STOC:BLPRS13})} 
Let $n$, $m$, and $q$ be positive integers and let $\mathcal{D}_{\mathbf{\Psi}_{\sigma}}^{m}$ be a discrete Gaussian distribution with noise rate parameter $\sigma > 2 \sqrt{n}$.  Then there exists a quantum reduction from worst-case $\left(n, \tilde{O} \left( n q / \sigma  \right) \right)-GapSVP$ to $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{U} \left( Z_{q}^{n} \right), \mathcal{D}_{\mathbf{\Psi}_{\sigma}} \right)$-LWE.  In addition, if $q \geq 2^{n/2}$, then there is also a classical reduction between those problems. 
\end{theorem}

We note that our presentation of this theorem differs quite a bit from the presentation in~\cite{STOC:BLPRS13} because they present LWE as a problem over the cycle (the additive group of reals modulo 1) for ease of exposition about the noise parameters, but it makes more sense when working in quantum money setting to present things over the integers.

\subsection{Helpful LWE Lemmas}
In this section, we add in some useful lemmas that allow us to change the distribution of the key in the LWE problem ($\mathcal{D}_{\rv}$) without affecting the hardness of the underlying problem too much.  Looking ahead, we will need to use various versions of the powerful modulus switching lemma from~\cite{STOC:BLPRS13}, which requires LWE instances with ``low-norm'' keys.

We start with a simple folklore lemma, which informally states that LWE with a uniformly sampled random key is at least as hard as LWE with any other secret key distribution.

\begin{lemma}~\label{lem:unifkey}
Let $n$, $m$, and $q$ be integers, let $\mathcal{D}_{\Am}$ and $\mathcal{D}_{\rv}$ be distributions over $\Z_{q}^{n}$, and let $\mathcal{D}_{\mathbb{\Psi}}$ be a distribution over $\Z_{q}^{m}$.  Any adversary that can solve the $\left(n, m, q, \mathcal{D}_{\Am}, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE problem with advantage $\epsilon$ can be used to solve the $\left(n, m, q, \mathcal{D}_{\Am}, \mathcal{D}_{\rv}, \mathcal{D}_{\mathbb{\Psi}} \right)$-LWE problem with advantage $\epsilon$.
\end{lemma}

\begin{proof}
We give an abbreviated proof because this result is simple and well-known.  Given an LWE challenge tuple $\left(\Am, \tv \right)$ where $\tv = \Am \cdot \rv + \ev$ and $\rv \leftarrow \mathcal{D}_{\rv}$ or $\tv$ is random, sample $\rv' \in \Z_{q}^{n}$ uniformly at random and add $\Am \cdot \rv'$ to $\tv$.  This gives the correct LWE distribution with a uniform key.
\end{proof}

We will also use a lemma from~\cite{STOC:BLPRS13} that says, informally speaking, that LWE with certain parameters where the key is drawn from the noise distribution is at least as hard as when the key is uniform (modulo some small parameter losses).  We state this below.

\begin{lemma}~\label{lem:noisekey} \textbf{(Lemma 2.12,~\cite{STOC:BLPRS13})}
Let $n$, $m$, and $q$ be positive integers with $q \geq 25$.  Let $m' = m - \left(16 n + 4 \ln \ln q \right)$.  Consider some parameter $s \geq \sqrt{\ln \left( 2n \left( 1 + 1/\epsilon \right) / \pi \right)}$.  Let $\epsilon < \frac{1}{2}$ and $\sigma, \sigma' > 0$ be real numbers such that $\sigma'  \geq \sqrt{ \sigma^{2} + s^{2}}$.  Finally, let $\mathcal{D}_{\mathbf{\Psi}_{\sigma}}$ be a discrete Gaussian distribution with parameter $\sigma$.

Any adversary that can solve the $\left(n, m', q, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbf{\Psi}_{\sigma'}}, \mathcal{D}_{\mathbf{\Psi}_{\sigma}} \right)$-LWE problem with advantage $\epsilon'$ can be used to solve the $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\mathbf{\Psi}_{\sigma}} \right)$-LWE problem with advantage $\left(\epsilon' - 8 \epsilon \right) / 4$.  In particular, assuming $\sigma > s$, we can take $s = \sigma$ and set $\sigma' = \sqrt{2} \sigma$.
\end{lemma}

Note that this lemma causes us to have to decrease the number of LWE samples we receive slightly (i.e. $m$ decreases) but does not change the dimension of the LWE problem ($n$).

\subsection{Modulus Switching}
In their seminal work~\cite{STOC:BLPRS13}, Brakerski \emph{et al.} use a technique called \emph{modulus switching} to improve known reductions from the GapSVP problem to the LWE problem.  Informally speaking, this modulus switching technique allows those authors to show that LWE in ``small modulus'' and ``high dimension'' is roughly equivalent in hardness to LWE in ``big modulus'' and ``low dimension''.  We state some of their results here since we would eventually like to use the fact that one-dimensional LWE with exponential modulus is hard, which is known from results in~\cite{STOC:BLPRS13}.

Rather than present a single instance of their main theorem, we go through two of their corollaries to make it easier to follow.  We emphasize that our presentation looks very different from theirs because they consider LWE over the unit cycle $\mathbb{T}$ and we work over the integers.

\begin{lemma}~\label{lem:modreduction} \textbf{(Corollary 3.2,~\cite{STOC:BLPRS13})}
Let $n$, $m$, $q$, and $q'$ be positive integers with $q' > q$, and consider some $\left(B, \delta \right)$-bounded distribution $\tilde{\mathcal{D}}$ over $\Z^{n}$.  Let $\epsilon \in \left(0, \frac{1}{2} \right)$ be a parameter and let $\sigma, \sigma > 0$ be real numbers.  Finally, let 
\[
\sigma' \geq \sqrt{ \left( \sigma \frac{q'}{q} \right)^{2} + \left(4 / \pi \right) \ln \left( 2n \left(1 + 1/ \epsilon \right) \right) \cdot B^{2} }
\]
Then there is an efficient reduction from $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \tilde{\mathcal{D}}, \mathcal{D}_{\mathbf{\Psi}_{\sigma}} \right)$ to $\left(n, m, q', \mathcal{U} \left( \Z_{q}^{n} \right), \tilde{\mathcal{D}}, \mathcal{D}_{\mathbf{\Psi}_{\sigma'}} \right)$ that reduces the advantage by at most $\sigma + 14 \epsilon m$. 
\end{lemma}

Informally speaking, this lemma gives us a way to reduce the modulus of an LWE instance while keeping the ``gap between the noise level and the modulus'' almost the same.  This is a rather counterintuitive result, and even moreso when you consider the fact that it works for essentially arbitrary distributions on LWE secrets.

We next present another modulus switching lemma that lets us go from ``high modulus, low dimension'' to ``normal modulus, normal dimension'' instances of LWE.  

\begin{lemma}~\label{lem:modexp} \textbf{(Corollary 3.4,~\cite{STOC:BLPRS13})}
Consider any positive integers $n$, $m$, $q$, and $k$ such that $k$ divides $n$, real numbers $\sigma, \sigma' > 0$, a parameter $\epsilon \in \left(0, \frac{1}{2} \right)$, and some $\left(B, \delta \right)$-bounded distribution $\tilde{\mathcal{D}}$.  In addition, let
\[
\sigma' \geq \sqrt{ \left( \sigma q^{k - 1} \right)^{2} + \left(4 / \pi \right) \ln \left( 2n \left(1 + 1/ \epsilon \right) \right) \cdot \left(B q^{k - 1}\right)^{2} }
\]
and define $\Gm = \mathbf{I}_{n/k} \otimes \left(1, q, q^{2}, ... , q^{k - 1} \right)^{T}$.

Then there is an efficient reduction from $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \tilde{\mathcal{D}}, \mathcal{D}_{\mathbf{\Psi}_{\sigma}} \right)$-LWE to $\left(n/k, m, q^{k}, \mathcal{U} \left( \Z_{q}^{n} \right), \tilde{\mathcal{D}}, \mathcal{D}_{\mathbf{\Psi}_{\sigma'}} \right)$-LWE that reduces the advantage by at most $\delta + 14 \epsilon m$.
\end{lemma}

Note that setting $k = n$ gives us hardness for single-dimension LWE (i.e. $n = 1$).

\subsection{The $k$-LWE Problem}
With the LWE definition in place, we are ready to move to the actual $k$-LWE problem.  The $k$-LWE problem was first formally defined in~\cite{C:LPSS14} and used to build traitor-tracing schemes.  It extends the $k$-SIS assumption~\cite{PKC:BonFre11} which was used to build linearly homomorphic signatures.  Our definition below is essentially a parameterized version of the one in~\cite{C:LPSS14}.

\begin{definition}~\label{def:kLWE} \textbf{$k$-LWE Problem:}
Let $k$, $n$, $m$, and $p$ be integers, let $\mathcal{D}_{\Rm}$ be a distribution over $\Z_{q}^{n}$, and let $\mathcal{D}_{\mathbb{\Psi}}$ and $\mathcal{D}_{\Sm}$ be distributions over $\Z_{q}^{m}$.  Let $\Sm \in \Z_{q}^{k \times m}$ be a matrix where each \emph{row} is selected from $\mathcal{D}_{\Sm}$.  

Let $\Am \in \Z_{q}^{m \times n}$ be a matrix sampled uniformly from the set of matrices such that $\Sm \cdot \Am = 0 \mod q$, let $\rv \in \Z_{q}^{n}$ be a vector sampled from $\mathcal{D}_{\rv}$, and let $\ev \in \Z_{q}^{m}$ be a vector sampled from $\mathcal{D}_{\mathbb{\Psi}}$.  Let $\Cm \in \Z_{q}^{m \times \left(m - k \right)}$ be a basis for the set of vectors $\vv \in \Z_{q}^{m}$ such that $\vv^{T} \cdot \Cm = 0$, and let $\rv' \in \Z_{q}^{m - k}$ be a uniformly random vector.

The $\left(k, n, m, q, \mathcal{D}_{\Sm}, \mathcal{D}_{\rv}, \mathcal{D}_{\mathbb{\Psi}} \right)$-$k$-LWE problem is defined to be distinguishing between the following distributions: 
\[  \left( \Sm, \Am, \Cm, \Am \cdot \rv+ \ev \right) \text{ and } \left(\Sm, \Am,  \Cm, \Cm \cdot \rv'+ \ev \right) \] 
\end{definition}

We note that $k$-LWE is traditionally defined in a slightly different way:  usually the matrix $\Am$ is sampled before (or jointly with) $\Sm$ rather than after it.  We sample $\Sm$ first in our definition because we will need to handle very unusual (at least for cryptographic applications) distributions $\mathcal{D}_{\Sm}$.

The authors of~\cite{C:LPSS14} prove the following theorem about $k$-LWE:

\begin{theorem}~\label{thm:oldkLWE} \textbf{(Theorem 3,~\cite{C:LPSS14})}:
Let $n$, $m$, and $p$ be integers, and $\sigma$ and $\sigma'$ be rational numbers such that $\sigma \geq \Omega \left(n \right)$, $\sigma' \geq \Omega \left(n^{3} \sigma^{2} / \log n \right)$, $p \geq \Omega \left( \sigma' \sqrt{\log m} \right)$ is prime, and $m \geq \Omega \left( n \log p \right)$.  For instance, we could set $\sigma = \Theta \left(n \right)$, $\sigma' = \Theta \left(n^{5} / \log n \right)$, $p = \Theta \left( n^{5} \right)$, and $m = \Theta \left( n \log n \right)$.  Let $\mathcal{D}_{alpha}^{d}$ and $\mathcal{D}_{\alpha'}^{d}$ denote discrete Gaussian distributions over $\Z^{d}$ with parameter $\alpha$ and $\alpha'$, respectively.

Define the matrix 
\[
\tilde{\Sm} = \left[ \begin{array}{cc}
\sigma \cdot \mathbf{I}_{m + n} & 0 \\
0 & \sigma' \cdot \mathbf{I}_{n}
\end{array} \right]
\]
and let $\mathcal{D}_{\tilde{\Sm}}$ denote the discrete Gaussian distibution over $\Z^{m + 2n}$ with skew $\tilde{\Sm}$.

Then, for some constant $c$ such that $k = n / \left(c \log n \right)$, there exists a PPT reduction from $\left(n, m+1, p, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\alpha} \right)$-LWE to $\left(k, n, m + 2n, p, \mathcal{D}_{\tilde{\Sm}}, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\alpha'} \right)$-k-LWE and advantage $\epsilon' = \Omega \left( \left( \epsilon - 2^{\Omega \left(n / \log n \right)} \right)^{3} - O \left(2^{-n} \right) \right)$.
\end{theorem}

Informally speaking, this theorem shows that $k$-LWE is hard for a fixed lattice dimension $n$ with only a minor (polynomial) blowup in parameters for a short vector distribution of a certain type of (nicely) skewed Gaussian.  Unfortunately, this distribution of short vectors is not related to the distribution implied by the~\cite{KLS22} scheme, so we cannot directly apply this theorem.  However, we will prove a different result than can directly be applied to the~\cite{KLS22} scheme.

\subsection{$k$-LWE for a Constant Number of Vectors Is Hard}
In this section we prove that $k$-LWE with the appropriate parameters is as hard as regular LWE for \emph{any} distribution on the short vectors, up to a superpolynomial loss in the noise, \emph{assuming that the number of short vectors $k$ is constant}.  We state this below.  Our proof is inspired by the $k$-SIS proof of~\cite{PKC:BonFre11}.

\begin{lemma}~\label{lem:constkLWE}
Let $k$, $n$, $m$, and $q$ be positive integers, and let $\mathcal{D}_{\Rm}$ be a distribution over $\Z_{q}^{n}$.  Let $\mathcal{D}_{\mathbb{\Psi}_{\sigma}}$ be a discrete Gaussian distribution over $\Z_{q}^{m}$ with noise parameter (width) $\sigma$.  Furthermore, let $\mathcal{D}_{\Sm}$ be a distributions over $\Z_{q}^{m}$ with the additional requirement that $\mathcal{D}_{\Sm}$ is $B$-bounded.  Let $\Sm \in \Z_{q}^{k \times m}$ be a matrix where each \emph{row} is selected from $\mathcal{D}_{\Sm}$.  Let $f \left(n \right)$ be a function that is superpolynomial in $n$.

Any adversary that can solve the $\left(k, n, m + k, q, \mathcal{D}_{\Sm}, \mathcal{D}_{\rv}, \mathcal{D}_{\mathbb{\Psi}_{\sigma f \left(n \right) }} \right)$-$k$-LWE problem with advantage $\epsilon$ can be used to solve the $\left(n, m, q, \mathcal{U} \left( \Z_{q}^{n} \right), \mathcal{D}_{\rv}, \mathcal{D}_{\mathbb{\Psi}_{\sigma}} \right)$-LWE problem with advantage $\epsilon - \negl \left(n \right)$.
\end{lemma}

\begin{proof}
Suppose we are given an LWE challenge tuple in the form of $\left(\Am, \tv \right)$ where $\tv = \Am \cdot \rv + \ev$ (the ``real'' case) or $\tv = \rv$ for some uniformly sampled $\rv$.  We will show that we can use this LWE challenge to build a $k$-LWE challenge of the appropriate distribution in a way that succeeds with all but negligible probability.  Thus, given an appropriate $k$-LWE adversary, we can simply feed it our challenge tuple and then mimic that response in the LWE challenge game, winning with probability negligibly close to $\epsilon$.  Our reduction proceeds as follows (and borrows heavily from the techniques of~\cite{PKC:BonFre11}): 

First, suppose we sample $\Sm \leftarrow \mathcal{D}_{\Sm} \in \Z_{q}^{k \times \left(m + k \right)}$ and let $\Sm_{i, j}$ denote the $\left(i, j \right)th$ entry of $\Sm$.  Suppose we pick $k$ columns of $\Sm$ such that the $k \times k$ submatrix formed by these columns is full-rank; and note that we can always do this unless $\Sm$ has rank less than $k$ (in which case, we can just reduce $\Sm$ by one row and repeat the process).  Call this matrix $\Tm$.  Let $\tilde{\Tm}$ denote the \emph{adjugate} matrix of $\Tm$; in other words, $\tilde{\Tm} \cdot \Tm = det \left( \Tm \right) \cdot \mathbf{I}_{k}$ and $\tilde{\Tm} \in \Z^{k \times k}$.  Let $\tilde{\Sm} \in \Z_{k \times m} = \tilde{\Tm} \cdot \Sm$, and note that it has the following structure:
\[
\tilde{\Sm} = \left[ \begin{array}{cccccccc}
det \left( \Tm \right) & 0 & 0 &... & 0 &\tilde{\Sm}_{1, k+1} & ... & \tilde{\Sm}_{1, k + m} \\
0 & det \left( \Tm \right) & 0 & ... &  0 & \tilde{\Sm}_{2, k + 1} & ... & \tilde{\Sm}_{2, k + m} \\
0 & 0 &  det \left( \Tm \right) & ... &  0 & \tilde{\Sm}_{3, k + 1} & ... & \tilde{\Sm}_{3, k + m} \\
... & ... & ... & ... & ... & ... & ... & ... \\
0 & 0 & 0 & ... &  det \left( \Tm \right) & \tilde{\Sm}_{k, k + 1} & ... & \tilde{\Sm}_{k, k + m} 
\end{array} \right]
\]
Suppose we let $\Um \in \Z^{\left(m + k \right) \times m}$ be defined in the following way:  for each entry $\Um_{i, j}$ where $i \leq k$, we set $\Um_{i,j} = \tilde{\Sm}_{i, j + k}$.  For each entry $\Um_{i, j}$ for $i > k$, we set $\Um_{i, j } = - det \left( \Tm \right)$ if $i = j$ and $0$ otherwise.  Note that, pictorially, this gives us the following structure:
\[
\Um = \left[ \begin{array}{ccccc}
\tilde{\Sm}_{1, k+1} & \tilde{\Sm}_{1, k+2} & \tilde{\Sm}_{1, k+3} & ... & \tilde{\Sm}_{1, k + m} \\
\tilde{\Sm}_{2, k + 1} & \tilde{\Sm}_{2, k + 2} & \tilde{\Sm}_{2, k + 3} &   ... & \tilde{\Sm}_{2, k + m} \\
\tilde{\Sm}_{3, k + 1} & \tilde{\Sm}_{3, k + 2} & \tilde{\Sm}_{3, k + 3} & ... & \tilde{\Sm}_{3, k + m} \\
 ... & ... & ... & ... & ... \\
 \tilde{\Sm}_{k, k + 1} &  \tilde{\Sm}_{k, k + 2} &  \tilde{\Sm}_{k, k + 3} &  ... & \tilde{\Sm}_{k, k + m} \\
- det \left( \Tm \right) & 0 & 0 &... & 0 \\
0 & - det \left( \Tm \right) & 0 & ... &  0  \\
0 & 0 & - det \left( \Tm \right) & ... & 0 \\
... & ... & ... & ... & ...\\
0 & 0 & 0 & ... & - det \left( \Tm \right)  
\end{array} \right]
\]
We interrupt the reduction to make a couple of claims.

\medskip
\noindent \textbf{Claim:  $\Sm \cdot \Um = 0$}.  This follows from the fact that $\tilde{\Sm}$ is orthogonal to $\Um$ by definition and $\Sm = \tilde{T} \Sm$.  Since $\Tm$ is invertible (over both $\Z$ and $\Z_{q}$, $\Sm \cdot \Um = 0$ if and only if $\tilde{\Sm} \cdot \Um = 0$.

\medskip
\noindent \textbf{Claim:  no entry in $\Um$ has value larger than $\left(2B \right)^{k}$}.  First, note that the determinant of any $k \times k$ matrix with entries in $\left[-B, B \right]$ is at most $\left(2B \right)^{k}$, and the determinant of any $B$-bounded smaller matrices must be smaller than that.  Since the entries of the adjugate matrices are themselves determinats of submatrices of $\Tm$, they must also follow this bound. 

\medskip

Now we may continue with our reduction.  Suppose we sample $\ev' \leftarrow \mathcal{D}_{\mathbb{\Psi}_{\sigma f \left(n \right)}}^{m + k}$ and let $\Am' \in \Z_{q}^{m + k} \times n = \Um \cdot \Am$ and $\tv' = \Um \cdot \tv + \ev'$.  Additionally, suppose we sample some random matrix $\Wm \in \Z_{q}^{m \times m}$ and set $\Cm = \Um \cdot \Wm$.  We claim that the tuple $\left(\Sm, \Am', \Cm, \tv' \right)$ is an appropriately distributed $k$-LWE challenge.  We show this in a number of claims:  first, with some claims that apply to both the ``real'' and ``random'' cases, and then we argue these cases separately.

\medskip
\noindent \textbf{Claim:  $\Cm$ is a uniform basis of the kernel of $\Sm$ $\mod q$.}  This follows from the fact that $\Sm \cdot \Cm = 0$ over $\Z$ and the ranks of the matrices sum to $m + k$.

\medskip
\noindent \textbf{Claim:  $\Am' = \Um \cdot \Am \mod q$ is distributed uniformly at random subject to the constraint $\Sm \cdot \Am' = 0$}.  Since $\Am$ is uniformly random and $\Um$ is a basis for all vectors in the kernel of $\Sm$, we know that $\Am'$ is distributed appropriately $\mod q$.

\medskip

So, at this point we know that $\Sm$, $\Am'$, and $\Cm$ are distributed appropriately.  All that remains is to handle $\tv'$  We handle this separately for the ``real'' and ``random'' cases below.

\medskip
\noindent \textbf{The ``Real'' Case.}  Assume now that $\tv = \Am \cdot \rv + \ev$.  Then we have 
\[
\tv' = \Um \left( \Am \cdot \rv + \ev \right) + \ev' = \Am' \cdot \rv + \left(\Um \ev + \ev' \right).
\]

If $k$ is constant, then $\left(2B \right)^{k}$ is constant and $\Um \ev$ has no entries larger than $O \left( m^2 \sigma \right)$ with all but negligible probability since the probability that a discrete Gaussian with parameter $\sigma$ is larger than $m \sigma$ is negligible.  Since $f \left(n \right)$ grows faster than any polynomial, we know that $\Um \cdot \ev + \ev'$ is distributed statistically close to just sampling a discrete Gaussian with parameter $\sigma f \left(n \right)$ (i.e. how we sampled $\ev'$), so we know that $\tv'$ is sampled appropriately in this case.  

\medskip
\noindent \textbf{The ``Random'' Case.}  Now assume that $\tv'$ is distributed uniformly at random over $\Z_{q}^{m}$.  In this case, we know that $\Um \cdot \tv$ is distributed uniformly at random over the kernel of $\Sm$ $\mod q$ and thus can be written as $\Cm \cdot \rv'$ for a uniformly random $\rv'$ as desired.  Since $\tv' = \Um \cdot \tv + \ev'$, we therefore know that the output distribution is correct in the ``random'' case as well.

\medskip

Completing these two cases finishes the reduction and completes the proof.
\end{proof}

\subsection{Putting It All Together}
In order to show that any adversary that can solve the $k$-LWE instance implied by the~\cite{KLS22} scheme can solve worst-case lattice problems, we just need to put all of our lemmas together.  Below, we show a table containing all of our hybrid arguments with approximate factors:  we ignore constant factors in the dimensions and polynomial factors in the noise and modulus (when the modulus is exponentially large).  We assume $q > \left(q' \right)^{n}$ and that the noise distributions are Gaussians.  We note that the ``Noise'' entry for GapSVP is the approximation ratio defined by the problem, not the noise itself.
\[
\begin{array}{|c|c|c|c|c|c|c|}
\text{Assumption} & \text{Lattice Dim.} & \text{Samples} & \text{Modulus} & \text{Key Dist.} & \text{Noise} & \text{Proof Comment} \\ \hline
k-LWE & 1 & m & q & \text{Unif.} & \frac{q}{\eta} & \text{n/a} \\ \hline
LWE & 1 & m & q & \text{Unif.} & \frac{q}{\eta f \left(n \right)} & \text{Lemma~\ref{lem:constkLWE}} \\ \hline
LWE & 1 & m & q & \text{Noise} & \frac{q}{\eta f \left(n \right)} & \text{Lemma~\ref{lem:unifkey}} \\ \hline
LWE & 1 & m & \left(q' \right)^{n} & \text{Noise} & \frac{\left(q' \right)^{n}}{\eta f \left(n \right)} & \text{Lemma~\ref{lem:modreduction}} \\ \hline
LWE & n & m & q' & \text{Noise} & \frac{q'}{\eta f \left(n \right)} & \text{Lemma~\ref{lem:modexp}} \\ \hline 
LWE & n & m & q' & \text{Unif.} & \frac{q'}{\eta f \left(n \right)} & \text{Lemma~\ref{lem:noisekey}} \\ \hline
GapSVP & n & - & - &  - & \eta f \left(n \right) & \text{Theorem~\ref{thm:LWEHardness}} \\ \hline
\end{array}
\]

We can state this in a nice lemma.

\begin{lemma}
Let $n$, $m$, $q$, and $k$ be integers such that $k$ is a constant.   Let $f \left(n \right)$ be some function that grows superpolynomially in $n$.  Let $q$ be exponentially large and $m$ polynomially sized in some security parameter $n$, and let $q' = poly \left(n \right) f \left(n \right)$.  Let $\sigma$ be a discrete Gaussian parameter such that $\sigma \geq \frac{q}{\eta}$ and let $\mathcal{D}_{\Psi_{\sigma}}$ denote a discrete Gaussian with parameter $\sigma$.  Let $\mathcal{D}_{\Sm}$ be any distribution over $\Z^{m}$ that outputs vectors bounded by some polynomial in $n$.

An adversary that solves the $\left(k, 1, m, q, \mathcal{D}_{\Sm}, \mathcal{U} \left( \Z_{q} \right), \mathcal{D}_{\Psi_{\sigma}} \right)$-k-LWE problem with non-negligible advantage can be used to solve the $\left( \log_{q'} \left(q \right), \sigma f \left(n \right) \right)$-GapSVP problem with non-negligible advantage.
\end{lemma}

\begin{proof}
The proof follows from a simple hybrid argument outlined in the table above.
\end{proof}

Note that $\log_{q'} \left(q \right)$ will be quite large (possibly even polynomial, depending on the choice of $q$), so the Gap-SVP problem reduced from here seems very likely to be hard.

==> transpage.tex <==
\newpage

\
\vfil
\hfil {\Huge Supplementary Material} \hfil
\vfil

\newpage
